Improved Network Calculus Delay Bounds in Time-Sensitive Networks

In time-sensitive networks, bounds on worst-case delays are typically obtained by using network calculus and assuming that flows are constrained by bit-level arrival curves. However, in IEEE TSN or IETF DetNet, source flows are constrained on the number of packets rather than bits. A common approach to obtain a delay bound is to derive a bit-level arrival curve from a packet-level arrival curve. However, such a method is not tight: we show that better bounds can be obtained by directly exploiting the arrival curves expressed at the packet level. Our analysis method also obtains better bounds when flows are constrained with g-regulation, such as the recently proposed Length-Rate Quotient rule. It can also be used to generalize some recently proposed network-calculus delay-bounds for a service curve element with known transmission rate.

==> lineShaping.tex <==
\section{Improvement on Flow Regulations}\label{sec:regimprov}
We can further improve the flow arrival curve and apply the theorems of Section \ref{sec:delay}.
%\begin{itemize}
%    \item impact of delay-jitter on bit-level and packet level arrival curves
%    \item impact of line-shaping on bit-level and packet-level arrival curves
%    \item impact of packetizer on bit-level and packet-level arrival curves
%\end{itemize}


\begin{itemize}
	\item line-shaping
	\item delay-jitter
	\item packetizer
\end{itemize}
